Model Counting meets F0 Estimation

Constraint satisfaction problems (CSP's) and data stream models are two powerful abstractions to capture a wide variety of problems arising in different domains of computer science. Developments in the two communities have mostly occurred independently and with little interaction between them. In this work, we seek to investigate whether bridging the seeming communication gap between the two communities may pave the way to richer fundamental insights. To this end, we focus on two foundational problems: model counting for CSP's and computation of zeroth frequency moments ($F_0$) for data streams. Our investigations lead us to observe striking similarity in the core techniques employed in the algorithmic frameworks that have evolved separately for model counting and $F_0$ computation. We design a recipe for translation of algorithms developed for $F_0$ estimation to that of model counting, resulting in new algorithms for model counting. We then observe that algorithms in the context of distributed streaming can be transformed to distributed algorithms for model counting. We next turn our attention to viewing streaming from the lens of counting and show that framing $F_0$ estimation as a special case of #DNF counting allows us to obtain a general recipe for a rich class of streaming problems, which had been subjected to case-specific analysis in prior works. In particular, our view yields a state-of-the art algorithm for multidimensional range efficient $F_0$ estimation with a simpler analysis.

==> counting2.tex <==
\section{From Streaming to Counting}
As a first step, we present a unified view of the three hashing-based algorithms proposed in Bar-Yossef et al. 

Algorithm~\ref{alg:hashstream}, called $\ComputeFZero$,  presents the overarching architecture of the three proposed algorithms. Each of these algorithms first pick up appropriate set of hash functions $H$  and initialize the set $\mathcal{S}$. 
The core architecture of {\ComputeFZero} is fairly simply:  it terminates at the end of the stream. For every element of the stream, {\ComputeFZero} simply calls the subroutine {\ProcessUpdate} which performs update depending on the type of estimation algorithm. In case of Bucketing, the subroutine {\UpdateHashAndSet} also updates the set of hash functions and $\mathcal{S}$. Finally, for each of the algorithms, we compute estimate based on the sketch $S$ and the set of hash functions $H$.  The corresponding steps for estimate computation are described in the subroutine {\ComputeEst}, presented as Algorithm. 
\begin{algorithm}[htb]
	\caption{$\ComputeFZero$}
	\label{alg:hashstream}
	\begin{algorithmic}[1]
		\State $H \gets \PickHashFunctions$
		\State $\mathcal{S} \gets \{\}$
		\While{true}
		%			\While{$\CheckUntil(S)$}
		\If{$\EndStream$} exit;
		\EndIf
		\State $x \gets input()$
		\State $\ProcessUpdate(\mathcal{S}, H, x)$
		%			\EndWhile
		\State $\UpdateHashAndSet(H, \mathcal{S})$
		\EndWhile
		\State $Est \gets \ComputeEst(H, \mathcal{S})$
		\State \Return $Est$
	\end{algorithmic}
\end{algorithm}

\begin{algorithm}
	\caption{$\ProcessUpdate(\mathcal{S}, H, x)$}
	\begin{algorithmic}[1]
		\For {$i \in [1, |H|$]}
		\Switch{AlgorithmType}
		\Case{Minimum}
		\State $j \gets argmax(S[i])$
		\If {$\mathcal{S}[i][j] > H[i](x)$}
		\State $\mathcal{S}[i][j]  \gets  min(\mathcal{S}[i][j],H[i](x))$
		\EndIf
		\EndCase		
		\Case{Estimation}
		
		\State $S[i] \gets min (S[i], \TrailZero(H[i](x)))$
		
		\EndCase		
		\Case{Bucketing}
		\If {$H[i](x) == 0$}
		\State $\mathcal{S}[i] \gets \mathcal{S}[i] \cup \{x\}$
		\EndIf
		\EndCase
		\EndSwitch	
		\EndFor 
		\State \Return $\mathcal{S}$
	\end{algorithmic}
\end{algorithm}

%\begin{algorithm}
% \caption{$\CheckUntil(S)$}
% \begin{algorithmic}[1]
% 	\If {AlgorithmType == Bucketing}
%		\If {$|S| = \frac{c}{\varepsilon^2}$}
%		\State \Return  True
%		\EndIf
% 	\EndIf
% 	\State \Return False
% \end{algorithmic}
%\end{algorithm}

\begin{algorithm}
	\caption{$\UpdateHashAndSet(H, \mathcal{S})$}
	\begin{algorithmic}[1]
		\If {AlgorithmType == Bucketing}
		\State $\thresh \gets \frac{48}{\varepsilon^2}$
		\For {$i \in [1, |H|$]}
		\If {$|\mathcal{S}[i]| = \thresh$}
		\State \IncrementRange($H[i])$
		\For{$x \in \mathcal{S}$}
		\If {$H[i](x) \neq 0$}
		\State Remove($\mathcal{S}[i], x$)
		\EndIf	
		\EndFor
		
		\EndIf
		\EndFor
		\EndIf
	\end{algorithmic}
\end{algorithm}

%\begin{algorithm}
%	\caption{$\ComputeEst(H,\mathcal{S})$}
%	\begin{algorithmic}[1]
%		
%	\end{algorithmic}
%\end{algorithm}

We now show how each of the three algorithms presented in Section can be transformed to corresponding algorithms for model counting. The recipe for such a transformation is based on the following insight: 

	\begin{enumerate}
		\item Capture the relationship $\mathcal{P} (\mathcal{S}, H, \mathbf{a}_{u})$ between the sketch $\mathcal{S}$, set of hash functions $H$, and unique set $\mathbf{a}_{u}$ at the end of stream. 
		\item The formula $\varphi$ is viewed as symbolic representation of the unique set $\mathbf{a}_{u}$ represented by the stream $\mathbf{a}$. 
		\item Given a formula $\varphi$ and set of hash functions $H$, design an algorithm to construct sketch $\mathcal{S}$ such that $\mathcal{P} (\mathcal{S}, H, \satisfying{\varphi})$ holds. 
	\end{enumerate}
	
\subsection{Minimum Value-based Algorithm}
For a given stream $\mathbf{a}$, the sketch $\mathcal{S}$ satisfies the following condition, $\mathcal{P}_1(\mathcal{S}, H, \mathbf{a}_{u})$. 
\begin{enumerate}
	\item $\forall i, |\mathcal{S}[i]|  = \min(\frac{96}{\varepsilon^2}, |\mathbf{a}_{u}| )$
	\item $\forall i, \forall y \notin \mathcal{S}[i],  \exists y' \in \mathcal{S}[i] \text{ such that} H[i](y') \preceq H[i](y)$
\end{enumerate}

Therefore, we can transform the minimum value-based algorithm for $F_0$ estimation to that of model counting given access to a subroutine that can compute $\mathcal{S}$ such that $\mathcal{P}_1(\mathcal{S}, H, \satisfying{\varphi})$ holds true. The following proposition establishes the existence and complexity of such a  subroutine, called {\FindMin}:
\begin{proposition}\label{prop:findmin}
Given $\varphi$ over $n$ variables, $h \in H_{xor}(n,m)$, and $t$ as input, there is an algorithm, {\FindMin}, that returns a set, $\mathcal{B}$ ,  of satisfying assignments  of $\varphi$ such that 
\begin{enumerate}
	\item $|\mathcal{B}| = min(t, |\satisfying{\varphi}|)$
	\item $\forall y \not\in \mathcal{B}$,  $\exists y' \in \mathcal{B}$ such that $h(y') \preceq h(y)$. 
\end{enumerate}
If $\varphi$ is a CNF formula, then {\FindMin} makes $\mathcal{O}(t\cdot m)$ calls to an NP oracle. If $\varphi$ is a DNF formula with $k$ terms, then {\FindMin} takes $\mathcal{O}(m^3 \cdot n \cdot k \cdot t)$ time. 
\end{proposition}

Equipped with Proposition~\ref{prop:findmin}, we are now ready to present the algorithm, called {\ApproxModelCountMin}, for model counting. Since the complexity of {\FindMin} is PTIME when $\varphi$ is in DNF, we have {\ApproxModelCountMin} as a FPRAS for DNF formulas. 

\begin{lemma}\label{lm:approxmin}
	Given $\varphi$, $\varepsilon$,$ \delta$, {\ApproxModelCountMin} returns $c$ such that $\Pr [ \frac{|\satisfying{\varphi}}{1+\varepsilon} \leq c \leq (1+\varepsilon)|\satisfying{\varphi}|] \geq 1- \delta$. {\ApproxModelCountMin} makes $\mathcal{O}(\frac{1}{\varepsilon^2}  m \log (\frac{1}{\delta}))$ calls to NP oracle. If $\varphi$ is a DNF formula, then {\ApproxModelCountMin} is an FPRAS. 
\end{lemma}




\begin{algorithm}
		\caption{$\ApproxModelCountMin (\varphi,\varepsilon, \delta)$}
		\label{alg:approxmin}
		\begin{algorithmic}[1]
			\State $H\gets \PickHashFunctions$
			\State $S \gets \{\}$
			\State $\thresh \gets \frac{c}{\varepsilon^2}$
			\For {$i \in  [1, |H|] $}
				\State $S[i] \gets \FindMin(\varphi, H[i], \thresh)$
			\EndFor
		
			\State $Est \gets \frac{1}{S[\thresh]}$
			\State \Return $Est$
		\end{algorithmic}
\end{algorithm}

\input{min}
\subsection{Estimation-based Algorithm}

We now turn to {\em estimation-based} algorithm  presented in Bar-Yoseff et al. For a given stream $\mathbf{a}$ and chosen hash functions $H$,
 the sketch $\mathcal{S}$ corresponding to estimation-based algorithm satisfies the relation $\mathcal{P}(\mathcal{S}, H, \mathbf{a}_u)$
 such that
 
 \begin{align}
 \mathcal{P}_{2}(\mathcal{S}, H, \mathbf{a}_u) := \left(S[i] = \min_{x \in \mathbf{a}_{u}} LeastZero(H[i])(x)\right)
 \end{align}

Following the recipe outlined above, we can transform a $F_0$ streaming algorithm to model counting algorithm by designing a subroutine that can compute the sketch for the set of all solutions described by $\varphi$. The following proposition describes a subroutine {\FindMaxRange}, which achieves the desired objective:


\begin{proposition}\label{prop:range}
	Given $\varphi$ over $n$ variables, $h \in H_{s}(n,n)$, there is an algorithm, {\FindMaxRange},  that returns $t$ such that 
	\begin{enumerate}
		\item $\exists z, z \models \varphi$ and $h(z)$ has $t$ least significant bits equal to zero. 
		\item $\forall (z \models \varphi h(z)) \implies $ $h(z)$ has $ \leq t$ least significant bits equal to zero. 
	\end{enumerate}
	If $\varphi$ is a CNF formula, then {\FindMaxRange} makes $\mathcal{O}(\log n)$ calls to NP oracle. If $\varphi$ is a DNF formula with $k$ terms, then {\FindMaxRange} is ?? \todo{KSM: @Arnab: Can you please look into it. }. \todo{We need proof for this}
\end{proposition}

Equipped with Proposition~\ref{prop:range}, we obtain {\ApproxModelCountEst} that takes in a formula $\varphi$
 and returns $|\satisfying{\varphi}|$. The key idea of {\ApproxModelCountEst} is to repeatedly invoke {\FindMaxRange} for each of the chosen hash functions and compute the estimate based on the sketch $\mathcal{S}$.  The following lemma summarizes the time complexity and guarantees of {\ApproxModelCountEst}
 
 \begin{lemma}\label{lm:est}
 	Given $\varphi$, $\varepsilon$,$ \delta$, {\ApproxModelCountEst} returns $c$ such that $\Pr [ \frac{|\satisfying{\varphi}}{1+\varepsilon} \leq c \leq (1+\varepsilon)|\satisfying{\varphi}|] \geq 1- \delta$. {\ApproxModelCountEst} makes $\mathcal{O}(\frac{1}{\varepsilon^2} \log M \log (\frac{1}{\delta}))$ calls to NP oracle. \todo{M needs to be figured out}
 \end{lemma}


\begin{algorithm}
	\caption{$\ApproxModelCountEst(\varphi,\varepsilon, \delta)$}
	\label{alg:approxest}
	\begin{algorithmic}[1]
		\State $H \gets \PickHashFunctions$
		\State $S \gets \{\}$
		\For {$i \in  [1, |H|] $}
		\State $S[i] \gets \FindMaxRange(\varphi, \TrailZero(H[i]))$
		\EndFor
		
		\State $Est \gets $
		\State \Return $Est$
	\end{algorithmic}
\end{algorithm}



\input{bucketing}

==> minOld.tex <==
\subsubsection{Implementing the Min-based Algorithm}

We now give a proof of Proposition~\ref{prop:findmin} by giving an implementation of  {\FindMin} subroutine. 


\begin{proof}

We present the algorithm when the formula $\varphi$ is a DNF formula. Adapting the algorithm for the case of CNF is straightforward. Our goal is to compute a set $\mathcal{B}$ of $t$ of satisfying assignments whose hashed values are lexicographically minimum among the hashed values of all  satisfying assignments of $\varphi$. 

Let $\phi = T_1\vee T_2\vee\ \cdots \vee T_k$ be a DNF formula over
$n$ variables where $T_i$ is a term. Let $h:\{0,1\}^n\rightarrow
\{0,1\}^{m}$  be a linear hash function in $\mathcal{H}_{xor}(n,m)$
defined by a $m\times n$ binary matrix $A$.  Let $\mathcal{C}$ be the set of hashed values of the
satisfying assignments for $\varphi$: $\mathcal{C} = \{h(x) \mid x \models \varphi\}
\subseteq \{0,1\}^m$. Let $\mathcal{C}_{t}$ be the first $t$
elements of $\mathcal{C}$ in the lexicographic order. By keeping the pair $(x,h(x))$: the solution $x$ and its hashed value, the task of computing $\mathcal{B}$ is same as computing $\mathcal{C}_t$. 

%\begin{theorem}
%There is an algorithm that takes a DNF formula $\Phi$ with $m$ terms
%on $n$ variables, a $N\times n$ binary matrix, and a number $t$ outputs
%$S_{\leq t}$ in time $O(N^3nmt)$ time.
%\end{theorem}

We will give an algorithm with running time $O(m^3nt)$ 
to compute $\mathcal{C}_t$ when the formula is just a
term $T$. Using this algorithm we can compute $\mathcal{C}_t$
for a formula with $k$ terms by iteratively merging $\mathcal{C}_t$ for each term. The time
complexity increases by a factor of $k$, resulting in an $O(m^3nkt)$ time algorithm.

Let $T$ be a term with width $w$ (number of literals) and $\mathcal{C} = \{Ax
\mid x \models T\}$. By fixing the variables in $T$ we get a vector $b_T$ and an $N\times
(n-w)$ matrix $A_T$ so that $S = \{A_Tx + b_T \mid x\in
\{0,1\}^{(n-w)}\}$. Both $A_T$ and $b_T$ can be computed
from $A$ and $T$ in linear time. Let  $h_T(x)$ be the transformation $A_Tx + b_T$. 

We will compute $\mathcal{C}_t$ ($t$ lexicographically minimum elements in $\mathcal{C}$) iteratively as follows: assuming we have computed $(q-1)^{th}$ minimum of $\mathcal{C}$, we will compute $q^{th}$ minimum using a prefix-searching strategy. We will use  a subroutine to solve the following basic prefix-searching primitive: Given any $l$ bit string $y_1\ldots y_l$, is there an $x\in \{0,1\}^{n-w}$ so that $y_1\ldots y_l$ is a prefix for some string in $\{h_T(x)\}$? This task can be performed using Gaussian elimination over an $(l+1)\times (n-w)$ binary matrix and can be implemented in time $O(l^2(n-w))$.  

Let $y=y_1\ldots y_m$ be the $(q-1)^{th}$ minimum in $\mathcal{C}$. Let $r_1$ be the rightmost 0 of $y$. Then using the above mentioned procedure we can find the lexicographically smallest string in the range of $h_T$ that extends $y_1\ldots y_{(r-1)}1$ if it exists. If no such string exists in $\mathcal{C}$,  find the index of the next   0 in $y$ and repeat the procedure.  In this manner the $q^{th}$ minimum can be computed using $O(m)$ calls to the prefix-searching primitive resulting in an $O(m^3n)$ time algorithm. Invoking the above procedure $t$ times results in an algorithm to compute $\mathcal{C}_t$ in $O(m^3nt)$ time.  

If $\varphi$ is a CNF formula, we can employ the same prefix searching strategy. Consider the following NP oracle: $O=\{\langle \varphi, h, y, y' \rangle \mid \exists x, \exists y'', \mbox{ so that } x \models \varphi, y'y'' > y,  h(x) = y'y'' \}$. With $m$ calls to $O$, we can compute string in $\mathcal{C}$ that is lexicographically greater than $y$. So with $t\cdot m$, calls to $O$, we can compute $\mathcal{C}_t$. 

\end{proof}
%
%\end{document}


==> streaming.tex <==
%\section{Hashing-based Schemes for $F_0$ Streaming}






==> weightedtorange.tex <==
\subsection*{From Weighted \#DNF  to d-Dimensional Ranges}

Consider a formula $\varphi$ defined on the set of variables $X = \{x_1, x_2, \ldots  x_n  \}$. Let a weight function $\rho: X \mapsto (0,1)$ 
such that weight of an assignment $\sigma \in 2^X$ can be defined as follows: 
\begin{align*}
W(\sigma) = \prod_{x_i \in \sigma} \rho(x_i) \prod_{x_i \notin \sigma} (1-\rho(x_i))
\end{align*} 
Furthermore, we define the weight of a formula $F$ as 
\begin{align*}
W(\varphi) = \sum_{\sigma \models \varphi} W(\sigma)
\end{align*}

Given $\varphi$ and $\rho$, the problem of weighted counting is to compute $W(F)$. We consider the case where for each $x_i$, $\rho(x_i)$ is represented using $m_i$ bits in binary representation, i.e., $\rho(x_i) = \frac{k_i}{2^{m_i}}$. Inspired by the key idea of weighted to unweighted reduction due to Chakraborty et al~\cite{CFMV15}, we show how the problem of weighted counting can be reduced to that of estimation of $F_0$ estimation of multi-dimensions ranges when $\varphi$ is a DNF formula. The reduction is as follows: we transform every term of $\varphi$ into a product of multi-dimension ranges where every variable $x_i$ is replaced with interval $[1,k_i]$ while $\neg x_i$ is replaced with $[k_i+1, 2^{m_i}]$ and every $\wedge$ is replaced with $\times. $
For example, a term $(x_1 \wedge \neg x_2 \wedge \neg x_3)$ is replaced with $[1,k_1]\times[k_2+1, 2^{m_2}]\times[k_3+1,2^{m_3}]$. Given $F_0$ of the resulting stream, we can compute the weight of $\varphi$ simply as $ W(\varphi) = \frac{F_0}{2^{\sum_i m_i} }$
%
%Our reduction allows us to use hashing-based technique proposed in for estimation of $F_0$, thereby resolving the open problem of whether there exists a hashing-based FPRAS for weighted DNF~\cite{ACL19}. Formally, 
%
%\begin{theorem}
%There exists a hashing-based FPRAS that takes in a formula $\varphi$, tolerance parameter $\varepsilon > 0$, confidence parameter $\delta > 0$ and returns an estimate $c$ such that 
%\begin{align*}
%\Pr[  \frac{W(\varphi)}{1+\varepsilon} \leq c \leq (1+\varepsilon) W(\varphi)   ] \geq 1-\delta
%\end{align*}
%
%
%\end{theorem}
